3-Dimensional CryoEM Pose Estimation and Shift Correction Pipeline

Accurate pose estimation and shift correction are key challenges in cryo-EM due to the very low SNR, which directly impacts the fidelity of 3D reconstructions. We present an approach for pose estimation in cryo-EM that leverages multi-dimensional scaling (MDS) techniques in a robust manner to estimate the 3D rotation matrix of each particle from pairs of dihedral angles. We express the rotation matrix in the form of an axis of rotation and a unit vector in the plane perpendicular to the axis. The technique leverages the concept of common lines in 3D reconstruction from projections. However, common line estimation is ridden with large errors due to the very low SNR of cryo-EM projection images. To address this challenge, we introduce two complementary components: (i) a robust joint optimization framework for pose estimation based on an $\ell_1$-norm objective or a similar robust norm, which simultaneously estimates rotation axes and in-plane vectors while exactly enforcing unit norm and orthogonality constraints via projected coordinate descent; and (ii) an iterative shift correction algorithm that estimates consistent in-plane translations through a global least-squares formulation. While prior approaches have leveraged such embeddings and common-line geometry for orientation recovery, existing formulations typically rely on $\ell_2$-based objectives that are sensitive to noise, and enforce geometric constraints only approximately. These choices, combined with a sequential pipeline structure, can lead to compounding errors and suboptimal reconstructions in low-SNR regimes. Our pipeline consistently outperforms prior methods in both Euler angle accuracy and reconstruction fidelity, as measured by the Fourier Shell Correlation (FSC).

==> sec/0_abstract.tex <==
\begin{abstract}
\textcolor{red}{many rotation matrices -- one per particle} Accurate pose estimation and shift correction from noisy 2D projections are fundamental challenges in cryo-electron microscopy (Cryo-EM), directly impacting the fidelity of 3D reconstructions. We present an approach for pose estimation in cryo-EM that leverages multi-dimensional scaling (MDS) techniques in a robust manner to estimate the rotation matrix of each projection from pairs of dihedral angles. We express the rotation matrix in the form of an axis of rotation and a unit vector in the plane perpendicular to the axis. The technique leverages the concept of common lines in 3D reconstruction from projections. However, common line estimation is ridden with large errors due to the very low SNR of cryo-EM projection images. To address this challenge, we introduce two complementary components: (i) a robust joint optimization framework for pose estimation based on an $\ell_1$-norm objective or a similar robust norm, which simultaneously estimates normal and in-plane vectors while exactly enforcing unit norm and orthogonality constraints via projected coordinate descent; and (ii) an iterative shift correction algorithm that estimates consistent in-plane translations through a global least-squares formulation. 
While prior approaches have leveraged spherical embeddings and common-line geometry for orientation recovery, existing formulations typically rely on $\ell_2$-based objectives that are sensitive to noise and enforce geometric constraints only approximately. These choices, combined with a sequential pipeline structure, can lead to compounding errors and suboptimal reconstructions in low-SNR regimes. Our pipeline consistently outperforms prior methods in both Euler angle accuracy and reconstruction fidelity, as measured by Fourier Shell Correlation (FSC). 
\end{abstract}


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{wacv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/1_introduction.tex <==
\section{Introduction}
Cryo-electron microscopy (Cryo-EM) has revolutionized structural biology by enabling near-atomic resolution imaging of biological macromolecules \cite{Frank2018}. It circumvents the need for crystallization, making it especially valuable for large or flexible complexes. In Cryo-EM, thousands of copies of a macromolecule (e.g., virus, ribosome, etc.) are put into a test-tube containing a solvent. The contents of the test-tube are poured onto a slide and frozen. The slide is imaged by a cryo-electron microscope which shoots electron beams vertically downwards on the slide and acquires an image called a `micrograph'. The micrograph contains the 2D projection images (called `particles') of each macromolecule copy in a random and unknown orientation, against a noisy background.
The particles are extracted from the noisy background via a technique called particle picking, which typically uses modern machine learning approaches \cite{Xu2025}. The core computational challenge lies in reconstructing the 3D structure from thousands of noisy particles, each of which has an unknown 3D orientation (a rotation matrix) and unknown 2D shift\footnote{Any shift in the $Z$ direction has no effect on the 2D projection.}. The unknown 2D shift is due to possible errors in locating the center of the particle during particle picking. Accurate pose estimation, i.e., recovering both orientation and in-plane rotation of each projection, is essential, as errors at this stage directly impact the fidelity of the final reconstruction.
Despite advances in computational methods, pose estimation remains challenging due to the extremely low signal-to-noise ratio (SNR) in projections and unknown translational shifts. 

If the underlying 3D structure is $f(x,y,z)$, then the $i$th projection image ($1\leq i\leq n$), corresponding to unknown 3D rotation matrix $\boldsymbol{R}_i \in \mathcal{SO}(3)$ and unknown shift $\boldsymbol{s}_i := (\Delta x_i,\Delta y_i,0)$, is given by:
\begin{equation}
h_i = \int f(\boldsymbol{R}^{\top}_i \boldsymbol{p} - \boldsymbol{s}_i) dz,    
\label{eq:projection}
\end{equation}
where $\boldsymbol{p} := (x,y,z)^{\top}$ is a spatial coordinate. The planes corresponding to projection images in different poses intersect in a single line called the `common line'. These common lines between different pairs of projection images carry information which is useful in estimating the unknown orientations $\{\boldsymbol{R}_i\}_{i=1}^n$ as has been exploited in several papers such as \cite{Vanheel_1981,singer2010detecting,muller2024algebraic}. Given a pair of projection images $h_i, h_j$ from different poses where $i \neq j$, the common line is essentially computed by finding the most similar pair of lines passing through the center of $h_i$ and $h_j$. Given a triple of projection images $h_i, h_j, h_k$ in different non-coplanar poses, the common lines between each pair helps determine the orientation of each projection image relative to the other via a method called angular reconstitution \cite{van1987angular}. However the low SNR of the particle images induces huge errors in the process of common line detection which adversely affects orientation estimation. Recent geometric approaches use global optimization over angular constraints via frameworks such as spherical embedding \cite{wang2024orientation,lu20223d} or synchronization matrices \cite{Shkolnisky2012_sync,wang2013_lud} to estimate projection orientations. However, these methods minimize $\ell_2$ losses that are sensitive to outliers, or enforce orthogonality of the rotation matrix only approximately. Moreover, these methods assume that the projections are pre-aligned (that is, they are centered and hence there are no shifts), limiting robustness in real-world scenarios. As we demonstrate later, our technique yields superior pose estimation results as compared to existing techniques such as \cite{lu2022,wang2013_lud,Shkolnisky2012_sync}.

There exist other methods such as RELION \cite{scheres2012relion} or Cryo-Sparc \cite{punjani2016building} which estimate the unknown structure $f$ and the pose parameters $\{\boldsymbol{R}_i, \boldsymbol{s}_i\}_{i=1}^n$ iteratively in an expectation-maximization (ExM) framework. However the emphasis in our work is on techniques that determine pose parameters first and use these as input for image reconstruction without the added feedback loop. This is along the lines of the ASPIRE toolbox for Cryo-EM\footnote{\url{http://spr.math.princeton.edu/}}. The advantage of such an approach is its simplicity. We also note that such an approach can be easily incorporated within an iterative ExM framework as a very principled initialization. 

% \subsection{Limitations of Existing Methods}
% Despite considerable progress, the following limitations persist:
% \begin{itemize}
%     \item \textbf{Sensitivity to noise:} Most approaches rely on $\ell_2$-norm losses, which amplify the influence of outliers in noisy data.
%     \item \textbf{Soft constraint enforcement:} Many methods treat geometric relationships as regularization terms rather than hard constraints, compromising physical accuracy.
%     \item \textbf{Sequential structure:} Decoupled pipelines can propagate and amplify early-stage errors.
%     \item \textbf{Computational inefficiency:} Optimization and deep models can be slow or impractical for large-scale datasets.
% \end{itemize}
The main contributions of our paper are:
\begin{itemize}[noitemsep]
\item A joint pose estimation framework using $\ell_1$-norm minimization over both dihedral and in-plane angles under hard (as they should be) orthogonality constraints.
\item A shift refinement method that enforces global consistency across projections via sparse linear equations derived from common lines.
\item Empirical validation on synthetic and real Cryo-EM datasets demonstrating improved orientation recovery and reconstruction quality over state-of-the-art baselines.
\end{itemize}
Our approach significantly improves Euler angle estimation accuracy and structural fidelity across simulated datasets, as evidenced by sharper Fourier Shell Correlation (FSC) curves \cite{van2005fourier} and reduced angular errors. 



==> sec/2_angle_estimation.tex <==
% \section{Angle estimation algorithm}

% We propose a refined three-stage embedding framework to estimate the orientations of projection images. Each projection is characterized by a unit normal vector and a corresponding in-plane axis, which jointly determine its orientation in 3D space. This orientation can be equivalently represented using Euler angles $(\alpha, \beta, \gamma)$, where $(\alpha, \beta)$ define the direction of the projection’s normal, and $\gamma$ captures the in-plane rotation around this axis.

% The complete algorithm consists of six core stages:

% \begin{enumerate}
%     \item \textbf{Common Line Detection:}  
%     For each pair of projection images, their mutual intersection in Fourier space—known as the common line—is determined. This relies on the central slice theorem, which asserts that the 2D Fourier transform of a projection lies on a central slice of the 3D Fourier volume. Normalized cross-correlation is used to identify the angle of intersection between projection pairs.

%     \item \textbf{Dihedral Angle Estimation:}  
%     For each image pair $(i, j)$, we estimate a dihedral angle $\theta_{ij}(k)$ using auxiliary projections $k \notin \{i,j\}$. Since these estimates are sensitive to noise in common line detection, a probabilistic voting mechanism is employed to enhance robustness:
%     \begin{equation}
%     \label{eq:voting_method}
%     \begin{split}
%     \text{hist}_{ij}(t) &= \sum_{k \ne i,j} 
%     \frac{1}{\sqrt{2\pi \sigma^2}} 
%     \exp\left( 
%     -\frac{(\sigma t - \theta_{ij}(k))^2}{2\sigma^2} 
%     \right), \notag \\
%     \sigma &= \frac{\pi}{T}, \quad t \in \{0, \ldots, T-1\} \notag \\
%     t_{\text{max}} &= \arg \max_t \text{hist}_{ij}(t) ,\\
%     W_{ij} &= \text{hist}_{ij}(t_{\text{max}}), \\
%     \theta_{ij} &= \sigma \cdot t_{\text{max}}
%     \end{split} 
%     \end{equation}
    
%     where $W_{ij}$ quantifies the confidence in the inferred angle.

%     \item \textbf{Initial Embedding of Normal Vectors:}  
%     With the estimated dihedral angles $\theta_{ij}$, we recover the projection normals by solving an L1-norm minimization:
%     \begin{equation}\label{eq:init_x}
%         \min_{D} \|W \odot (DD^T - \cos(\Theta/r))\|_1 \quad \text{s.t.} \quad \|d_i\|^2 = 1 \;\forall i
%     \end{equation}
%     where $D \in \mathbb{R}^{n \times 3}$ contains unit vectors representing the normal directions of projections.

%     \item \textbf{Estimation of In-Plane Relationships:}  
%     Given an initial estimate of the normal vectors $D^{(0)}$, we derive the relative in-plane angles through:
%     \begin{equation}
%         \cos(\Phi_{ij}) = \cos C_{ij} \cos C_{ji} + \sin C_{ij} \sin C_{ji} \cos(\theta_{ij}^{(E)})
%     \end{equation}
%     where $\theta_{ij}^{(E)} = \arccos((D^{(0)} (D^{(0)})^T)_{ij})$. The in-plane axes $Q$ are recovered by solving:
%     \begin{equation}
%         \min_Q \|W \odot (QQ^T - \cos(\boldsymbol{\Phi}))\|_1 \quad \text{s.t.} \quad \|q_i\|^2 = 1 \;\forall i
%     \end{equation}

%     \item \textbf{Initial Orthogonality Alignment:}  
%     To encourage orthogonality between normal vectors $D^{(0)}$ and the in-plane directions $Q^{(0)}$, we compute a rotation matrix $R \in SO(3)$ that minimizes:
%     \begin{equation}
%         \min_R \|\text{diag}(D^{(0)} R (Q^{(0)})^T)\|_2^2 \quad \text{s.t.} \quad R^T R = I_3
%     \end{equation}
%     The rotated in-plane directions are updated as $\tilde{Q}^{(0)} = Q^{(0)} R^T$, and the initializations are set as:
%     \begin{align}
%         D_0 &= D^{(0)} \\
%         Q_0 &= \tilde{Q}^{(0)}
%     \end{align}

%     \item \textbf{Joint Optimization:}  
%     Finally, we refine both $D$ and $Q$ through a joint optimization that enforces unit norm constraints and orthogonality between corresponding vectors:
%     \begin{equation}\label{eq:jointopt}
%     \begin{aligned}
%     \min_{D,Q} \quad & \|W \odot (DD^T - \cos(\Theta/r))\|_1 \\
%     & + \|W \odot (QQ^T - \cos(\boldsymbol{\Phi}))\|_1 \\
%     \text{s.t.} \quad & \|d_i\|_2 = 1,\quad \|q_i\|_2 = 1,\quad d_i^\top q_i = 0 \\
%     & \text{for } i = 1,\ldots,n
%     \end{aligned}
%     \end{equation}
    
    
%     where the third constraint enforces that $d_i^T q_i = 0$ for each projection $i$, ensuring perpendicularity of normal and in-plane axes.
% \end{enumerate}


% % \subsubsection{Optimization via Coordinate Descent}

% We solve the joint objective~\eqref{eq:jointopt} using a projected coordinate descent algorithm. The method alternates between updating $D$ and $Q$ while enforcing the unit norm and orthogonality constraints. $C_{ij}$ and $C_{ji}$ denote the angles between common lines and local coordinate axes.

% \paragraph{Gradient Computation}

% Let $Z_1 = \cos(\Theta/r)$ and define:
% \begin{equation}
% \begin{aligned}
% C &= \cos(C_{ij}), \quad S = \sin(C_{ij}), \\
% A_{ij} &= C \odot C^\top, \quad B_{ij} = S \odot S^\top.
% \end{aligned}
% \end{equation}

% We define the residuals:
% \begin{equation}
% R_D = W \odot (DD^\top - Z_1),
% \end{equation}
% \begin{equation}
% R_Q = W \odot \left( QQ^\top - \left( A_{ij} + B_{ij} \odot DD^\top \right) \right).
% \end{equation}

% The gradient updates are given by:
% \begin{equation} \label{eq:grad_x_clean}
% \begin{aligned}
% G_x =\ & 2(W \odot \text{sign}(R_D))D \\
% & - 2(W \odot B_{ij} \odot \text{sign}(R_Q))D,
% \end{aligned}
% \end{equation}
% \begin{equation} \label{eq:grad_y_clean}
% G_y = 2(W \odot \text{sign}(R_Q))Q.
% \end{equation}

% \paragraph{Constraint Projection}

% After each gradient step, constraints are enforced row-wise:
% \begin{equation}
% \begin{aligned}
% d_i &\leftarrow d_i - (d_i^\top q_i) q_i, \quad d_i \leftarrow \frac{d_i}{\|d_i\|_2}, \\
% q_i &\leftarrow q_i - (q_i^\top d_i) d_i, \quad q_i \leftarrow \frac{q_i}{\|q_i\|_2}.
% \end{aligned}
% \end{equation}

% \begin{algorithm}[H]
% \caption{Coordinate Descent for Joint Embedding}
% \begin{algorithmic}[1]
% \State \textbf{Initialize:} $D \leftarrow D_0$, $Q \leftarrow Q_0$
% \For{$k = 1,2,\dots,K_{\max}$}
%     \State Compute $C = \cos(C_{ij})$, $S = \sin(C_{ij})$
%     \State $A_{ij} \leftarrow C \odot C^\top$, $B_{ij} \leftarrow S \odot S^\top$
%     \State Compute residuals $R_D$, $R_Q$
%     \State Compute gradient $G_x$ using Eq.~\eqref{eq:grad_x_clean}
%     \State $D \leftarrow D - \alpha G_x$
%     \For{each $i$}
%         \State Project $d_i$ orthogonal to $q_i$ and normalize
%     \EndFor
%     \State Recompute $R_Q$, compute $G_y$ using Eq.~\eqref{eq:grad_y_clean}
%     \State $Q \leftarrow Q - \beta G_y$
%     \For{each $i$}
%         \State Project $q_i$ orthogonal to $d_i$ and normalize
%     \EndFor
%     \State Check convergence criteria
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% \subsection{Empirical validation}
% We validate our idea based on synthetically generated noisy projections from multiple 3D maps. We reconstruct a map using our pipeline and benchmark it against \cite{lu2022} to highlight the effectiveness of our angle estimation method. 


\section{Method}
\subsection{Common-line detection and voting method}
In ideal conditions, the Central Section Theorem states that the 2D Fourier transform of a projection image corresponds to a central slice through the 3D Fourier transform of the underlying structure, orthogonal to the projection direction. Consequently, the Fourier transforms of any two projections intersect along a common line. We estimate these common lines between image pairs via normalized cross-correlation~\cite{Vanheel_1981}.

Following this, dihedral angles between image pairs are estimated using the probabilistic voting strategy introduced in \cite{Singer2010}. For a given pair of projection images $(h_i, h_j)$, this method aggregates dihedral angle estimates $\theta_{ij}^{(k)}$ derived by involving a third image $h_k$ where $k \ne i,j$. Each choice of $k$ contributes a potentially noisy angle estimate. These estimates are combined into a smooth histogram using Gaussian kernels, with the peak of the histogram determining the final dihedral angle:
\begin{equation}
\theta_{ij} = \underset{t}{\arg\max}\dfrac{1}{n-2} \sum_{k \ne i,j} \frac{1}{\sqrt{2\pi\sigma^2}} \exp\left( -\frac{(\theta_{ij}^{(k)} - t)^2}{2\sigma^2} \right)
\end{equation}
where $\sigma := \pi/T$ controls the angular resolution. The height of the histogram peak also serves as a confidence score for the estimated dihedral angle. Compared to directly using common line angles, this voting-based aggregation improves reliability by mitigating the impact of inconsistent estimates due to noise.

\subsection{Joint Pose Estimation via Robust \texorpdfstring{$\ell_1$}{l1}-Norm Optimization}
For the rotation matrix $\boldsymbol{R}_i$, we denote its axis of rotation by $\boldsymbol{d}_i$ and the chosen X-axis of its local coordinate system (in the plane perpendicular to $\boldsymbol{d}_i$) by $\boldsymbol{q}_i$. Let $\boldsymbol{D} \in \mathbb{R}^{n \times 3}$ denote the matrix of rotation axes, and $\boldsymbol{Q} \in \mathbb{R}^{n \times 3}$ denote the matrix of in-plane X-axis vectors, one row per projection. The goal is to estimate these directions from noisy pairwise angular measurements derived from common lines. Let $\boldsymbol{\Theta} \in \mathbb{R}^{n \times n}$ denote the matrix of estimated dihedral angles between their rotation axes $\boldsymbol{d}_i$, and let $\boldsymbol{\Phi} \in \mathbb{R}^{n \times n}$ denote the matrix of angles between the in-plane local X-axis vectors. The weight matrix $\boldsymbol{W} \in \mathbb{R}^{n \times n}$ encodes the confidence in each pairwise measurement obtained as $W_{ij} :=  \underset{t}{\max}\dfrac{1}{n-2} \sum_{k \ne i,j} \frac{1}{\sqrt{2\pi\sigma^2}} \exp\left( -\frac{(\theta_{ij}^{(k)} - t)^2}{2\sigma^2} \right)$.  

Given pairwise common lines and dihedral angles, our aim is to estimate $\{\boldsymbol{R}_i\}_{i=1}^n$ through $\{\boldsymbol{d}_i\}_{i=1}^n$ and $\{\boldsymbol{q}_i\}_{i=1}^n$. In principle, this is akin to the technique of determining point coordinates from pairwise distances between the points \cite{singer2008remark}, which is the essence of the technique of multi-dimensional scaling (MDS) \cite{cox2008multidimensional}. However, for the specific problem at hand, the vectors $\{\boldsymbol{d}_i\}_{i=1}^n$ and $\{\boldsymbol{q}_i\}_{i=1}^n$ are constrained to lie on the unit sphere, so this a spherical embedding problem \cite{wilson2014}. Here, we jointly estimate $\boldsymbol{D}$ and $\boldsymbol{Q}$ by solving the following \emph{robust} optimization problem:
\begin{equation}
\begin{aligned}
\min_{\boldsymbol{D}, \boldsymbol{Q}} J(\boldsymbol{D}, \boldsymbol{Q}) := \quad & \|\boldsymbol{W} \odot (\boldsymbol{D}\boldsymbol{D}^\top - \cos(\boldsymbol{\Theta}))\|_1 \\
& \quad + \|\boldsymbol{W} \odot (\boldsymbol{Q}\boldsymbol{Q}^\top - \cos(\boldsymbol{\Phi}))\|_1 \\
\text{s.t.} \quad & \forall i, \|\boldsymbol{d}_i\|_2 = \|\boldsymbol{q}_i\|_2 = 1, \quad \boldsymbol{d}_i^\top \boldsymbol{q}_i = 0,
\end{aligned}
\label{eq:joint_opt}
\end{equation}
where $\odot$ denotes the Hadamard (element-wise) product. The cosine of in-plane angles is computed element-wise as:
\begin{equation}
\cos(\Phi_{ij}) = \cos C_{ij} \cos C_{ji} + \sin C_{ij} \sin C_{ji} \cdot (\boldsymbol{d}_i^\top \boldsymbol{d}_j),
\label{eq:phi_ij}
\end{equation}
as it is the dot product between the local X-axis vectors of $h_i$ and $h_j$ respectively given as $(\cos C_{ij}, \sin C_{ij},0)$ and $(\cos C_{ji}, \sin C_{ji} (\boldsymbol{d}_i^\top \boldsymbol{d}_j),\sin C_{ji} \sin \cos^{-1} (\boldsymbol{d}_i^\top \boldsymbol{d}_j))$.

Here, $C_{ij}$ and $C_{ji}$ (elements of the $n \times n$ matrix $\boldsymbol{C}$) are angles between the detected common lines and the chosen local X-axes of projections $i$ and $j$ respectively (computed from the particles directly). This formulation imposes exact orthogonality constraints and leverages the robustness of $\ell_1$ norms to handle outliers and inconsistencies in angular measurements, which are inevitable due to the low SNR.

\subsection{Initialization}
We adopt a two-step initialization strategy based on projected subgradient descent (PGD), enforcing unit norm constraints at each step:
\begin{enumerate}
    \item We initialize the normal vector matrix $\boldsymbol{D}^{(0)}$ by minimizing the first term in Eq.~\eqref{eq:joint_opt} using PGD, with projection onto the unit sphere after each update to enforce $\|\boldsymbol{d}_i\|_2 = 1$.
    \item Using the resulting $\boldsymbol{D}^{(0)}$, we compute $\cos(\Phi_{ij})$ from the common-line geometry via \eqref{eq:phi_ij} and initialize the in-plane vector matrix $\boldsymbol{Q}^{(0)}$ by minimizing the second term in Eq.~\eqref{eq:joint_opt}, again applying PGD with unit norm projection $\|\boldsymbol{q}_i\|_2 = 1$.
\end{enumerate}

To incentivize the orthogonality constraint $\boldsymbol{d}_i^\top \boldsymbol{q}_i = 0$, we apply a post-processing alignment step where we solve the following optimization problem:
\begin{equation}
\min_{\boldsymbol{R}^\top \boldsymbol{R} = \boldsymbol{I}} \left\| \operatorname{diag}(\boldsymbol{D}^{(0)} \boldsymbol{R} (\boldsymbol{Q}^{(0)})^\top) \right\|_2^2,
\end{equation}
to find an orthonormal matrix $\boldsymbol{R}$ and define the adjusted in-plane vectors as $\tilde{\boldsymbol{Q}}^{(0)} = \boldsymbol{Q}^{(0)} \boldsymbol{R}^\top$. The pair $(\boldsymbol{D}^{(0)}, \tilde{\boldsymbol{Q}}^{(0)})$ is then used as the initialization for the joint optimization problem where the orthogonality constraint is strictly enforced.

\subsection{Optimization via Coordinate Descent}
We solve the problem in \eqref{eq:joint_opt} using projected coordinate descent: alternating updates to $\boldsymbol{D}$ and $\boldsymbol{Q}$ with sub-gradient steps and projection onto the appropriate constraint sets.

\noindent\textbf{$\boldsymbol{D}$-update:} The gradient of the loss $J(.)$ with respect to $\boldsymbol{D}$ includes the sum of both terms from \eqref{eq:joint_opt}: one with $\boldsymbol{D}\boldsymbol{D}^\top$ and the other with $\cos (\boldsymbol{\Phi}))$ (since $\cos(\boldsymbol{\Phi})$ depends on $\boldsymbol{D}\boldsymbol{D}^\top$ as seen in \eqref{eq:phi_ij}). We define the following quantities which will help us arrive at the expression for $\nabla J_{\boldsymbol{D}}$:
\begin{align}
\boldsymbol{A} &:= \cos \boldsymbol{C} \cdot (\cos \boldsymbol{C})^\top \\
\boldsymbol{B} &:= \sin \boldsymbol{C} \cdot (\sin \boldsymbol{C})^\top \\
\boldsymbol{Z} &:= \boldsymbol{A} + \boldsymbol{B} \odot (\boldsymbol{D}\boldsymbol{D}^\top)\\
\boldsymbol{R}_{\boldsymbol{D}} &:= \boldsymbol{W} \odot (\boldsymbol{D}\boldsymbol{D}^\top - \cos(\boldsymbol{\Theta})) \\
\boldsymbol{R}_{\boldsymbol{Q}} &:= \boldsymbol{W} \odot (\boldsymbol{Q}\boldsymbol{Q}^\top - \boldsymbol{Z}).
\end{align}
This yields:
\begin{equation}
\nabla J_{\boldsymbol{D}} = 2(\boldsymbol{W} \odot \operatorname{sign}(\boldsymbol{R}_{\boldsymbol{D}}
))\boldsymbol{D} - 2(\boldsymbol{W} \odot \boldsymbol{B} \odot \operatorname{sign}(\boldsymbol{R}_{\boldsymbol{Q}}))\boldsymbol{D}.
\end{equation}
After each gradient descent update, we project each $\boldsymbol{d}_i$ to satisfy:
\begin{align}
\boldsymbol{d}_i &\leftarrow \boldsymbol{d}_i - (\boldsymbol{d}_i^\top \boldsymbol{q}_i) \boldsymbol{q}_i \quad \text{(orthogonalize)}, \\
\boldsymbol{d}_i &\leftarrow \frac{\boldsymbol{d}_i}{\|\boldsymbol{d}_i\|_2} \quad \text{(normalize)}.
\end{align}
\noindent\textbf{$\boldsymbol{Q}$-update:} Once $\boldsymbol{D}$ is updated, we recompute $\boldsymbol{Z}$ and apply the gradient descent to update $\boldsymbol{Q}$:
\begin{align}
\boldsymbol{R}_{\boldsymbol{Q}} &:= \boldsymbol{W} \odot (\boldsymbol{Q}\boldsymbol{Q}^\top - \boldsymbol{Z}) \\
\nabla J_{\boldsymbol{Q}} &= 2(\boldsymbol{W} \odot \operatorname{sign}(\boldsymbol{R}_{\boldsymbol{Q}}))\boldsymbol{Q}
\end{align}
Each $\boldsymbol{q}_i$ is similarly projected to satisfy $\boldsymbol{d}_i^\top \boldsymbol{q}_i = 0$ and $\|\boldsymbol{q}_i\|_2 = 1$.

The complete procedure is summarized in Alg.~\ref{alg:PGD}.
\begin{algorithm}
\caption{Joint Pose Estimation via Coordinate Descent}
\begin{algorithmic}[1]
\Require Initial $\boldsymbol{D}, \boldsymbol{Q}$, weight matrix $W$, learning rates $\alpha, \beta$
\For{$k = 1$ to $K_{\max}$}
    \State Compute $\boldsymbol{R}_{\boldsymbol{D}}$, $\boldsymbol{R}_{\boldsymbol{Q}}$, and gradients $\boldsymbol{\nabla}_{\boldsymbol{D}}$, $\boldsymbol{\nabla}_{\boldsymbol{Q}}$
    \State $\boldsymbol{D} \leftarrow \boldsymbol{D} - \alpha \nabla_{\boldsymbol{D}}$; enforce orthogonality and unit norm on each $\boldsymbol{d}_i$
    \State $\boldsymbol{Q} \leftarrow \boldsymbol{Q} - \beta \boldsymbol{\nabla}_{\boldsymbol{Q}}$; enforce orthogonality and unit norm on each $\boldsymbol{q}_i$
    \If{converged}
        \State \textbf{break}
    \EndIf
\EndFor
\State \textbf{return} $\boldsymbol{D}, \boldsymbol{Q}$
\end{algorithmic}
\label{alg:PGD}
\end{algorithm}

After the projection angles are estimated, the FIRM method \cite{wang2013} can be used to produce the final 3D reconstruction result.

% \begin{table}[h]
% \centering
% \caption{
% Pose estimation errors across three synthetic maps at SNR = 0.1 using 1000 projections. Each cell shows: \textbf{Ours / Baseline}, with the better value in bold. MAE: Mean Absolute Error, MSE: Mean Squared Error}
% \label{tab:synthetic_results}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Metric (type)} & \textbf{EMD-3508} & \textbf{EMD-42525} & \textbf{EMD-22689} \\
% \hline
% $\theta_{ij}$ error (MAE) & \textbf{0.0267} / 0.0747 & \textbf{0.00518} / 0.01008 & \textbf{0.2584} / 0.3667 \\
% \hline
% $\phi_{ij}$ error (MAE) & \textbf{0.0196} / 0.0795 & \textbf{0.00392} / 0.02995 & \textbf{0.1946} / 0.3457 \\
% \hline
% In-plane rotation error (°) & \textbf{1.56} / 6.56 & \textbf{0.20} / 2.01 & \textbf{21.19} / 31.47 \\
% \hline
% Normal vector error (°) & \textbf{1.59} / 4.74 & \textbf{0.32} / 0.60 & \textbf{17.58} / 27.72 \\
% \hline
% Euler angle error $\alpha$ (MSE) & \textbf{0.00081} / 0.00571 & \textbf{\boldmath$2.4\!\times\!10^{-5}$} / $7.0\!\times\!10^{-5}$ & \textbf{0.0246} / 0.0559 \\
% Euler angle error $\beta$ (MSE) & \textbf{0.00936} / 0.03943 & \textbf{\boldmath$7.8\!\times\!10^{-5}$} / $2.6\!\times\!10^{-4}$ & \textbf{0.6925} / 0.9536 \\
% Euler angle error $\gamma$ (MSE) & \textbf{0.00930} / 0.04331 & \textbf{\boldmath$6.4\!\times\!10^{-5}$} / $1.4\!\times\!10^{-3}$ & \textbf{0.5701} / 0.7725 \\
% \hline
% \end{tabular}
% }
% \end{table}

\begin{table*}[ht]
\centering
\caption{Pose estimation errors across three synthetic maps at SNR = 0.1 using 1000 projections. Each cell reports the metric values for \textbf{Ours / SE / LUD / Sync}, where SE refers to the standard spherical embedding~\cite{lu2022}. Best result per row is in \textbf{bold}. MAE: Mean Absolute Error, MSE: Mean Squared Error.}
\label{tab:synthetic_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Metric (type)} & \textbf{EMD-3508} & \textbf{EMD-42525} & \textbf{EMD-22689} \\
\hline
$\theta_{ij}$ error (MAE) 
& \textbf{0.0267} / 0.0747 / 0.3035 / 0.2024 
& \textbf{0.00518} / 0.01008 / 0.05196 / 0.05278 
& \textbf{0.2584} / 0.3667 / 0.3874 / 0.2624 \\
\hline
$\phi_{ij}$ error (MAE) 
& \textbf{0.0196} / 0.0795 / 0.1996 / 0.1643 
& \textbf{0.00392} / 0.02995 / 0.03510 / 0.04613 
& 0.1946 / 0.3457 / 0.2676 / \textbf{0.1933} \\
\hline
In-plane rotation error (°) 
& \textbf{1.56} / 6.56 / 17.52 / 12.64 
& \textbf{0.20} / 2.01 / 1.58 / 1.94 
& 21.19 / 31.47 / 21.71 / \textbf{19.58} \\
\hline
Normal vector error (°) 
& \textbf{1.59} / 4.74 / 17.70 / 12.64 
& \textbf{0.32} / 0.60 / 2.76 / 3.14 
& 17.58 / 27.72 / 23.55 / \textbf{15.59} \\
\hline
Euler angle error $\alpha$ (MSE) 
& \textbf{0.00081} / 0.00571 / 0.05001 / 0.04878 
& \textbf{2.4e-5} / 7.0e-5 / 3.55e-3 / 1.86e-3 
& \textbf{0.0246} / 0.0559 / 0.07472 / 0.04186 \\
\hline
Euler angle error $\beta$ (MSE) 
& \textbf{0.00936} / 0.03943 / 0.35182 / 0.14755 
& \textbf{7.8e-5} / 2.6e-4 / 7.29e-3 / 5.23e-3 
& 0.6925 / 0.9536 / 0.4925 / \textbf{0.4046} \\
\hline
Euler angle error $\gamma$ (MSE) 
& \textbf{0.00930} / 0.04331 / 0.30561 / 0.16116 
& \textbf{6.4e-5} / 1.4e-3 / 3.82e-3 / 2.29e-3 
& 0.5701 / 0.7725 / 0.3833 / \textbf{0.3788} \\
\hline
\end{tabular}
}
\end{table*}



\begin{figure*}
\centering
\includegraphics[width=0.59\linewidth]{wacv-2026-author-kit-template/Results/Without_shifts/Visual_Results_without_results_combined.png}
\includegraphics[width=\linewidth]{wacv-2026-author-kit-template/Results/Without_shifts/FSC_without_shifts_results_combined.png}
\caption{Visual Comparison and FSC curves for 1000 simulated centered particles of SNR 0.1 for 3 different maps. These results confirm that robust joint pose estimation not only improves angular consistency but also yields higher-quality reconstructions, even in the presence of strong noise.}
\label{fig:joint_opt_validation}
\end{figure*}


==> sec/2_angles_SAVED.tex <==
% \section{Angle estimation algorithm}

% We propose a refined three-stage embedding framework to estimate the orientations of projection images. Each projection is characterized by a unit normal vector and a corresponding in-plane axis, which jointly determine its orientation in 3D space. This orientation can be equivalently represented using Euler angles $(\alpha, \beta, \gamma)$, where $(\alpha, \beta)$ define the direction of the projection’s normal, and $\gamma$ captures the in-plane rotation around this axis.

% The complete algorithm consists of six core stages:

% \begin{enumerate}
%     \item \textbf{Common Line Detection:}  
%     For each pair of projection images, their mutual intersection in Fourier space—known as the common line—is determined. This relies on the central slice theorem, which asserts that the 2D Fourier transform of a projection lies on a central slice of the 3D Fourier volume. Normalized cross-correlation is used to identify the angle of intersection between projection pairs.

%     \item \textbf{Dihedral Angle Estimation:}  
%     For each image pair $(i, j)$, we estimate a dihedral angle $\theta_{ij}(k)$ using auxiliary projections $k \notin \{i,j\}$. Since these estimates are sensitive to noise in common line detection, a probabilistic voting mechanism is employed to enhance robustness:
%     \begin{equation}
%     \label{eq:voting_method}
%     \begin{split}
%     \text{hist}_{ij}(t) &= \sum_{k \ne i,j} 
%     \frac{1}{\sqrt{2\pi \sigma^2}} 
%     \exp\left( 
%     -\frac{(\sigma t - \theta_{ij}(k))^2}{2\sigma^2} 
%     \right), \notag \\
%     \sigma &= \frac{\pi}{T}, \quad t \in \{0, \ldots, T-1\} \notag \\
%     t_{\text{max}} &= \arg \max_t \text{hist}_{ij}(t) ,\\
%     W_{ij} &= \text{hist}_{ij}(t_{\text{max}}), \\
%     \theta_{ij} &= \sigma \cdot t_{\text{max}}
%     \end{split} 
%     \end{equation}
    
%     where $W_{ij}$ quantifies the confidence in the inferred angle.

%     \item \textbf{Initial Embedding of Normal Vectors:}  
%     With the estimated dihedral angles $\theta_{ij}$, we recover the projection normals by solving an L1-norm minimization:
%     \begin{equation}\label{eq:init_x}
%         \min_{D} \|W \odot (DD^T - \cos(\Theta/r))\|_1 \quad \text{s.t.} \quad \|d_i\|^2 = 1 \;\forall i
%     \end{equation}
%     where $D \in \mathbb{R}^{n \times 3}$ contains unit vectors representing the normal directions of projections.

%     \item \textbf{Estimation of In-Plane Relationships:}  
%     Given an initial estimate of the normal vectors $D^{(0)}$, we derive the relative in-plane angles through:
%     \begin{equation}
%         \cos(\Phi_{ij}) = \cos C_{ij} \cos C_{ji} + \sin C_{ij} \sin C_{ji} \cos(\theta_{ij}^{(E)})
%     \end{equation}
%     where $\theta_{ij}^{(E)} = \arccos((D^{(0)} (D^{(0)})^T)_{ij})$. The in-plane axes $Q$ are recovered by solving:
%     \begin{equation}
%         \min_Q \|W \odot (QQ^T - \cos(\boldsymbol{\Phi}))\|_1 \quad \text{s.t.} \quad \|q_i\|^2 = 1 \;\forall i
%     \end{equation}

%     \item \textbf{Initial Orthogonality Alignment:}  
%     To encourage orthogonality between normal vectors $D^{(0)}$ and the in-plane directions $Q^{(0)}$, we compute a rotation matrix $R \in SO(3)$ that minimizes:
%     \begin{equation}
%         \min_R \|\text{diag}(D^{(0)} R (Q^{(0)})^T)\|_2^2 \quad \text{s.t.} \quad R^T R = I_3
%     \end{equation}
%     The rotated in-plane directions are updated as $\tilde{Q}^{(0)} = Q^{(0)} R^T$, and the initializations are set as:
%     \begin{align}
%         D_0 &= D^{(0)} \\
%         Q_0 &= \tilde{Q}^{(0)}
%     \end{align}

%     \item \textbf{Joint Optimization:}  
%     Finally, we refine both $D$ and $Q$ through a joint optimization that enforces unit norm constraints and orthogonality between corresponding vectors:
%     \begin{equation}\label{eq:jointopt}
%     \begin{aligned}
%     \min_{D,Q} \quad & \|W \odot (DD^T - \cos(\Theta/r))\|_1 \\
%     & + \|W \odot (QQ^T - \cos(\boldsymbol{\Phi}))\|_1 \\
%     \text{s.t.} \quad & \|d_i\|_2 = 1,\quad \|q_i\|_2 = 1,\quad d_i^\top q_i = 0 \\
%     & \text{for } i = 1,\ldots,n
%     \end{aligned}
%     \end{equation}
    
    
%     where the third constraint enforces that $d_i^T q_i = 0$ for each projection $i$, ensuring perpendicularity of normal and in-plane axes.
% \end{enumerate}


% % \subsubsection{Optimization via Coordinate Descent}

% We solve the joint objective~\eqref{eq:jointopt} using a projected coordinate descent algorithm. The method alternates between updating $D$ and $Q$ while enforcing the unit norm and orthogonality constraints. $C_{ij}$ and $C_{ji}$ denote the angles between common lines and local coordinate axes.

% \paragraph{Gradient Computation}

% Let $Z_1 = \cos(\Theta/r)$ and define:
% \begin{equation}
% \begin{aligned}
% C &= \cos(C_{ij}), \quad S = \sin(C_{ij}), \\
% A_{ij} &= C \odot C^\top, \quad B_{ij} = S \odot S^\top.
% \end{aligned}
% \end{equation}

% We define the residuals:
% \begin{equation}
% R_D = W \odot (DD^\top - Z_1),
% \end{equation}
% \begin{equation}
% R_Q = W \odot \left( QQ^\top - \left( A_{ij} + B_{ij} \odot DD^\top \right) \right).
% \end{equation}

% The gradient updates are given by:
% \begin{equation} \label{eq:grad_x_clean}
% \begin{aligned}
% G_x =\ & 2(W \odot \text{sign}(R_D))D \\
% & - 2(W \odot B_{ij} \odot \text{sign}(R_Q))D,
% \end{aligned}
% \end{equation}
% \begin{equation} \label{eq:grad_y_clean}
% G_y = 2(W \odot \text{sign}(R_Q))Q.
% \end{equation}

% \paragraph{Constraint Projection}

% After each gradient step, constraints are enforced row-wise:
% \begin{equation}
% \begin{aligned}
% d_i &\leftarrow d_i - (d_i^\top q_i) q_i, \quad d_i \leftarrow \frac{d_i}{\|d_i\|_2}, \\
% q_i &\leftarrow q_i - (q_i^\top d_i) d_i, \quad q_i \leftarrow \frac{q_i}{\|q_i\|_2}.
% \end{aligned}
% \end{equation}

% \begin{algorithm}[H]
% \caption{Coordinate Descent for Joint Embedding}
% \begin{algorithmic}[1]
% \State \textbf{Initialize:} $D \leftarrow D_0$, $Q \leftarrow Q_0$
% \For{$k = 1,2,\dots,K_{\max}$}
%     \State Compute $C = \cos(C_{ij})$, $S = \sin(C_{ij})$
%     \State $A_{ij} \leftarrow C \odot C^\top$, $B_{ij} \leftarrow S \odot S^\top$
%     \State Compute residuals $R_D$, $R_Q$
%     \State Compute gradient $G_x$ using Eq.~\eqref{eq:grad_x_clean}
%     \State $D \leftarrow D - \alpha G_x$
%     \For{each $i$}
%         \State Project $d_i$ orthogonal to $q_i$ and normalize
%     \EndFor
%     \State Recompute $R_Q$, compute $G_y$ using Eq.~\eqref{eq:grad_y_clean}
%     \State $Q \leftarrow Q - \beta G_y$
%     \For{each $i$}
%         \State Project $q_i$ orthogonal to $d_i$ and normalize
%     \EndFor
%     \State Check convergence criteria
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% \subsection{Empirical validation}
% We validate our idea based on synthetically generated noisy projections from multiple 3D maps. We reconstruct a map using our pipeline and benchmark it against \cite{lu2022} to highlight the effectiveness of our angle estimation method. 


\section{Method}
\subsection{Common-line detection and voting method}
In ideal conditions, the Central Section Theorem states that the 2D Fourier transform of a projection image corresponds to a central slice through the 3D Fourier transform of the underlying structure, orthogonal to the projection direction. Consequently, the Fourier transforms of any two projections intersect along a common line. We estimate these common lines between image pairs via normalized cross-correlation~\cite{Vanheel_1981}.

Following this, dihedral angles between image pairs are estimated using the probabilistic voting strategy introduced in \cite{Singer2010}. For a given pair of projection images $(h_i, h_j)$, this method aggregates dihedral angle estimates $\theta_{ij}^{(k)}$ derived by involving a third image $h_k$ where $k \ne i,j$. Each choice of $k$ contributes a potentially noisy angle estimate. These estimates are combined into a smooth histogram using Gaussian kernels, with the peak of the histogram determining the final dihedral angle:
\begin{equation}
\theta_{ij} = \underset{t}{\arg\max}\dfrac{1}{n-2} \sum_{k \ne i,j} \frac{1}{\sqrt{2\pi\sigma^2}} \exp\left( -\frac{(\theta_{ij}^{(k)} - t)^2}{2\sigma^2} \right)
\end{equation}
where $\sigma := \pi/T$ controls the angular resolution. The height of the histogram peak also serves as a confidence score for the estimated dihedral angle. Compared to directly using common line angles, this voting-based aggregation improves reliability by mitigating the impact of inconsistent estimates due to noise.

\subsection{Joint Pose Estimation via Robust \texorpdfstring{$\ell_1$}{l1}-Norm Optimization}
For the rotation matrix $\boldsymbol{R}_i$, we denote its axis of rotation by $\boldsymbol{d}_i$ and the X-axis of its local coordinate system (in the plane perpendicular to $\boldsymbol{d}_i$) by $\boldsymbol{q}_i$ \alertKG{Can't we arbitrarily choose a local coordinate system?}. Let $\boldsymbol{D} \in \mathbb{R}^{n \times 3}$ denote the matrix of rotation axes, and $\boldsymbol{Q} \in \mathbb{R}^{n \times 3}$ denote the matrix of in-plane X-axis vectors, one row per projection. The goal is to estimate these directions from noisy pairwise angular measurements derived from common lines. Let $\boldsymbol{\Theta} \in \mathbb{R}^{n \times n}$ denote the matrix of estimated dihedral angles between their rotation axes $\boldsymbol{d}_i$, and let $\boldsymbol{\Phi} \in \mathbb{R}^{n \times n}$ denote the matrix of angles between the in-plane local X-axis vectors. The weight matrix $\boldsymbol{W} \in \mathbb{R}^{n \times n}$ encodes the confidence in each pairwise measurement obtained as $W_{ij} :=  \underset{t}{\max}\dfrac{1}{n-2} \sum_{k \ne i,j} \frac{1}{\sqrt{2\pi\sigma^2}} \exp\left( -\frac{(\theta_{ij}^{(k)} - t)^2}{2\sigma^2} \right)$.  

Given pairwise common lines and dihedral angles, our aim is to estimate $\{\boldsymbol{R}_i\}_{i=1}^n$ through $\{\boldsymbol{d}_i\}_{i=1}^n$ and $\{\boldsymbol{q}_i\}_{i=1}^n$. In principle, this is akin to the technique of determining point coordinates from pairwise distances between the points \cite{singer2008remark}, which is the essence of the technique of multi-dimensional scaling (MDS) \cite{cox2008multidimensional}. However, for the specific problem at hand, the vectors $\{\boldsymbol{d}_i\}_{i=1}^n$ and $\{\boldsymbol{q}_i\}_{i=1}^n$ are constrained to lie on the unit sphere, so this a spherical embedding problem \cite{wilson2014}. Here, we jointly estimate $\boldsymbol{D}$ and $\boldsymbol{Q}$ by solving the following \emph{robust} optimization problem:
\begin{equation}
\begin{aligned}
\min_{\boldsymbol{D}, \boldsymbol{Q}} J(\boldsymbol{D}, \boldsymbol{Q}) := \quad & \|\boldsymbol{W} \odot (\boldsymbol{D}\boldsymbol{D}^\top - \cos(\boldsymbol{\Theta}))\|_1 \\
& \quad + \|\boldsymbol{W} \odot (\boldsymbol{Q}\boldsymbol{Q}^\top - \cos(\boldsymbol{\Phi}))\|_1 \\
\text{s.t.} \quad & \forall i, \|\boldsymbol{d}_i\|_2 = \|\boldsymbol{q}_i\|_2 = 1, \quad \boldsymbol{d}_i^\top \boldsymbol{q}_i = 0,
\end{aligned}
\label{eq:joint_opt}
\end{equation}
where $\odot$ denotes the Hadamard (element-wise) product. The cosine of in-plane angles is computed element-wise as:
\begin{equation}
\cos(\Phi_{ij}) = \cos C_{ij} \cos C_{ji} + \sin C_{ij} \sin C_{ji} \cdot (\boldsymbol{d}_i^\top \boldsymbol{d}_j),
\label{eq:phi_ij}
\end{equation}
as it is the dot product between the local X-axis vectors of $h_i$ and $h_j$ respectively given as $(\cos C_{ij}, \sin C_{ij},0)$ and $(\cos C_{ji}, \sin C_{ji} (\boldsymbol{d}_i^\top \boldsymbol{d}_j),\sin C_{ji} \sin \cos^{-1} (\boldsymbol{d}_i^\top \boldsymbol{d}_j))$.

Here, $C_{ij}$ and $C_{ji}$ (elements of the $n \times n$ matrix $\boldsymbol{C}$) are angles between the detected common lines and the chosen local X-axes of projections $i$ and $j$ respectively (computed from the particles directly). This formulation imposes exact orthogonality constraints and leverages the robustness of $\ell_1$ norms to handle outliers and inconsistencies in angular measurements, which are inevitable due to the low SNR.

\subsection{Initialization}
We adopt a two-step initialization strategy based on projected subgradient descent (PGD), enforcing unit norm constraints at each step:
\begin{enumerate}
    \item We initialize the normal vector matrix $\boldsymbol{D}^{(0)}$ by minimizing the first term in Eq.~\eqref{eq:joint_opt} using PGD, with projection onto the unit sphere after each update to enforce $\|\boldsymbol{d}_i\|_2 = 1$.
    \item Using the resulting $\boldsymbol{D}^{(0)}$, we compute $\cos(\Phi_{ij})$ from the common-line geometry via \eqref{eq:phi_ij} and initialize the in-plane vector matrix $\boldsymbol{Q}^{(0)}$ by minimizing the second term in Eq.~\eqref{eq:joint_opt}, again applying PGD with unit norm projection $\|\boldsymbol{q}_i\|_2 = 1$.
\end{enumerate}

To incentivize the orthogonality constraint $\boldsymbol{d}_i^\top \boldsymbol{q}_i = 0$, we apply a post-processing alignment step where we solve the following optimization problem:
\begin{equation}
\min_{\boldsymbol{R}^\top \boldsymbol{R} = \boldsymbol{I}} \left\| \operatorname{diag}(\boldsymbol{D}^{(0)} \boldsymbol{R} (\boldsymbol{Q}^{(0)})^\top) \right\|_2^2,
\end{equation}
to find an orthonormal matrix $\boldsymbol{R}$ and define the adjusted in-plane vectors as $\tilde{\boldsymbol{Q}}^{(0)} = \boldsymbol{Q}^{(0)} \boldsymbol{R}^\top$. The pair $(\boldsymbol{D}^{(0)}, \tilde{\boldsymbol{Q}}^{(0)})$ is then used as the initialization for the joint optimization problem where the orthogonality constraint is strictly enforced.

\subsection{Optimization via Coordinate Descent}
We solve the problem in \eqref{eq:joint_opt} using projected coordinate descent: alternating updates to $\boldsymbol{D}$ and $\boldsymbol{Q}$ with sub-gradient steps and projection onto the appropriate constraint sets.

\noindent\textbf{$\boldsymbol{D}$-update:} The gradient of the loss $J(.)$ with respect to $\boldsymbol{D}$ includes the sum of both terms from \eqref{eq:joint_opt}: one with $\boldsymbol{D}\boldsymbol{D}^\top$ and the other with $\cos (\boldsymbol{\Phi}))$ (since $\cos(\boldsymbol{\Phi})$ depends on $\boldsymbol{D}\boldsymbol{D}^\top$ as seen in \eqref{eq:phi_ij}). We define the following quantities which will help us arrive at the expression for $\nabla J_{\boldsymbol{D}}$:
\begin{align}
\boldsymbol{A} &:= \cos \boldsymbol{C} \cdot (\cos \boldsymbol{C})^\top \\
\boldsymbol{B} &:= \sin \boldsymbol{C} \cdot (\sin \boldsymbol{C})^\top \\
\boldsymbol{Z} &:= \boldsymbol{A} + \boldsymbol{B} \odot (\boldsymbol{D}\boldsymbol{D}^\top)\\
\boldsymbol{R}_{\boldsymbol{D}} &:= \boldsymbol{W} \odot (\boldsymbol{D}\boldsymbol{D}^\top - \cos(\boldsymbol{\Theta})) \\
\boldsymbol{R}_{\boldsymbol{Q}} &:= \boldsymbol{W} \odot (\boldsymbol{Q}\boldsymbol{Q}^\top - \boldsymbol{Z}).
\end{align}
This yields:
\begin{equation}
\nabla J_{\boldsymbol{D}} = 2(\boldsymbol{W} \odot \operatorname{sign}(\boldsymbol{R}_{\boldsymbol{D}}
))\boldsymbol{D} - 2(\boldsymbol{W} \odot \boldsymbol{B} \odot \operatorname{sign}(\boldsymbol{R}_{\boldsymbol{Q}}))\boldsymbol{D}.
\end{equation}
After each gradient descent update, we project each $\boldsymbol{d}_i$ to satisfy:
\begin{align}
\boldsymbol{d}_i &\leftarrow \boldsymbol{d}_i - (\boldsymbol{d}_i^\top \boldsymbol{q}_i) \boldsymbol{q}_i \quad \text{(orthogonalize)}, \\
\boldsymbol{d}_i &\leftarrow \frac{\boldsymbol{d}_i}{\|\boldsymbol{d}_i\|_2} \quad \text{(normalize)}.
\end{align}
\noindent\textbf{$\boldsymbol{Q}$-update:} Once $\boldsymbol{D}$ is updated, we recompute $\boldsymbol{Z}$ and apply the gradient descent to update $\boldsymbol{Q}$:
\begin{align}
\boldsymbol{R}_{\boldsymbol{Q}} &:= \boldsymbol{W} \odot (\boldsymbol{Q}\boldsymbol{Q}^\top - \boldsymbol{Z}) \\
\nabla J_{\boldsymbol{Q}} &= 2(\boldsymbol{W} \odot \operatorname{sign}(\boldsymbol{R}_{\boldsymbol{Q}}))\boldsymbol{Q}
\end{align}
Each $\boldsymbol{q}_i$ is similarly projected to satisfy $\boldsymbol{d}_i^\top \boldsymbol{q}_i = 0$ and $\|\boldsymbol{q}_i\|_2 = 1$.

The complete procedure is summarized in Alg.~\ref{alg:PGD}.
\begin{algorithm}
\caption{Joint Pose Estimation via Coordinate Descent}
\begin{algorithmic}[1]
\Require Initial $\boldsymbol{D}, \boldsymbol{Q}$, weight matrix $W$, learning rates $\alpha, \beta$
\For{$k = 1$ to $K_{\max}$}
    \State Compute $\boldsymbol{R}_{\boldsymbol{D}}$, $\boldsymbol{R}_{\boldsymbol{Q}}$, and gradients $\boldsymbol{\nabla}_{\boldsymbol{D}}$, $\boldsymbol{\nabla}_{\boldsymbol{Q}}$
    \State $\boldsymbol{D} \leftarrow \boldsymbol{D} - \alpha \nabla_{\boldsymbol{D}}$; enforce orthogonality and unit norm on each $\boldsymbol{d}_i$
    \State $\boldsymbol{Q} \leftarrow \boldsymbol{Q} - \beta \boldsymbol{\nabla}_{\boldsymbol{Q}}$; enforce orthogonality and unit norm on each $\boldsymbol{q}_i$
    \If{converged}
        \State \textbf{break}
    \EndIf
\EndFor
\State \textbf{return} $\boldsymbol{D}, \boldsymbol{Q}$
\end{algorithmic}
\label{alg:PGD}
\end{algorithm}

After the projection angles are estimated, the FIRM method \cite{wang2013} can be used to produce the final 3D reconstruction result.

\section{Synthetic Validation of Joint Pose Estimation}
We evaluated the effectiveness of our joint $\ell_1$-norm based pose estimation on simulated Cryo-EM datasets corrupted with heavy noise \textcolor{red}{how much noise?}. Specifically, we use three molecular maps from the well known database EMDB from \url{https://www.ebi.ac.uk/emdb/}. We simulated projections of these macromolecules at different angles and added noise to as to produce a signal-to-noise ratio (SNR) of 0.1:
\begin{itemize}[noitemsep,topsep=0pt]
    \item \textbf{Map 1 (EMD-3508)} – 80S ribosome, size $260^3 \cite{emd3508_Huter2016}$
    \item \textbf{Map 2 (EMD-42525)} – 80S ribosome, size $648^3 \cite{emd42525_Musalgaonkar2025Reh1}$
    \item \textbf{Map 3 (EMD-22689)} – PTCH1 with nanobody, size $256^3 \cite{emd22689_pnas.2011560117}$
\end{itemize}
We generated 1000 Gaussian-corrupted projections per map and comparde our method to the spherical embedding approach (SE) ~\cite{lu2022}, least unsquared deviations (LUD)~\cite{wang2013_lud}, and synchronization-based pose estimation (Sync) ~\cite{Shkolnisky2012_sync}, using standard metrics for angular and reconstruction accuracy.
Table~\ref{tab:synthetic_results} reports errors for dihedral and in-plane angle consistency, in-plane rotation, and Euler angles. Figure~\ref{fig:joint_opt_validation} presents visual comparisons and Fourier Shell Correlation (FSC) curves for three synthetic maps. We observe that reconstructions generated using our joint optimization framework align more closely with the ground truth, both in terms of structural detail and frequency preservation, as indicated by higher FSC values across resolutions. In particular, for Map 3 (EMD-22689), it is clearly visible in Figure~\ref{fig:joint_opt_validation} that our method yields the most accurate 3D reconstruction among all baselines. These results confirm that robust joint pose estimation not only improves angular consistency but also leads to significantly better reconstructions, even under high noise conditions.



% \begin{table}[h]
% \centering
% \caption{
% Pose estimation errors across three synthetic maps at SNR = 0.1 using 1000 projections. Each cell shows: \textbf{Ours / Baseline}, with the better value in bold. MAE: Mean Absolute Error, MSE: Mean Squared Error}
% \label{tab:synthetic_results}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Metric (type)} & \textbf{EMD-3508} & \textbf{EMD-42525} & \textbf{EMD-22689} \\
% \hline
% $\theta_{ij}$ error (MAE) & \textbf{0.0267} / 0.0747 & \textbf{0.00518} / 0.01008 & \textbf{0.2584} / 0.3667 \\
% \hline
% $\phi_{ij}$ error (MAE) & \textbf{0.0196} / 0.0795 & \textbf{0.00392} / 0.02995 & \textbf{0.1946} / 0.3457 \\
% \hline
% In-plane rotation error (°) & \textbf{1.56} / 6.56 & \textbf{0.20} / 2.01 & \textbf{21.19} / 31.47 \\
% \hline
% Normal vector error (°) & \textbf{1.59} / 4.74 & \textbf{0.32} / 0.60 & \textbf{17.58} / 27.72 \\
% \hline
% Euler angle error $\alpha$ (MSE) & \textbf{0.00081} / 0.00571 & \textbf{\boldmath$2.4\!\times\!10^{-5}$} / $7.0\!\times\!10^{-5}$ & \textbf{0.0246} / 0.0559 \\
% Euler angle error $\beta$ (MSE) & \textbf{0.00936} / 0.03943 & \textbf{\boldmath$7.8\!\times\!10^{-5}$} / $2.6\!\times\!10^{-4}$ & \textbf{0.6925} / 0.9536 \\
% Euler angle error $\gamma$ (MSE) & \textbf{0.00930} / 0.04331 & \textbf{\boldmath$6.4\!\times\!10^{-5}$} / $1.4\!\times\!10^{-3}$ & \textbf{0.5701} / 0.7725 \\
% \hline
% \end{tabular}
% }
% \end{table}

\begin{table*}[ht]
\centering
\caption{Pose estimation errors across three synthetic maps at SNR = 0.1 using 1000 projections. Each cell reports the metric values for \textbf{Ours / SE / LUD / Sync}, where SE refers to the standard spherical embedding~\cite{lu2022}. Best result per row is in \textbf{bold}. MAE: Mean Absolute Error, MSE: Mean Squared Error.}
\label{tab:synthetic_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Metric (type)} & \textbf{EMD-3508} & \textbf{EMD-42525} & \textbf{EMD-22689} \\
\hline
$\theta_{ij}$ error (MAE) 
& \textbf{0.0267} / 0.0747 / 0.3035 / 0.2024 
& \textbf{0.00518} / 0.01008 / 0.05196 / 0.05278 
& \textbf{0.2584} / 0.3667 / 0.3874 / 0.2624 \\
\hline
$\phi_{ij}$ error (MAE) 
& \textbf{0.0196} / 0.0795 / 0.1996 / 0.1643 
& \textbf{0.00392} / 0.02995 / 0.03510 / 0.04613 
& 0.1946 / 0.3457 / 0.2676 / \textbf{0.1933} \\
\hline
In-plane rotation error (°) 
& \textbf{1.56} / 6.56 / 17.52 / 12.64 
& \textbf{0.20} / 2.01 / 1.58 / 1.94 
& 21.19 / 31.47 / 21.71 / \textbf{19.58} \\
\hline
Normal vector error (°) 
& \textbf{1.59} / 4.74 / 17.70 / 12.64 
& \textbf{0.32} / 0.60 / 2.76 / 3.14 
& 17.58 / 27.72 / 23.55 / \textbf{15.59} \\
\hline
Euler angle error $\alpha$ (MSE) 
& \textbf{0.00081} / 0.00571 / 0.05001 / 0.04878 
& \textbf{2.4e-5} / 7.0e-5 / 3.55e-3 / 1.86e-3 
& \textbf{0.0246} / 0.0559 / 0.07472 / 0.04186 \\
\hline
Euler angle error $\beta$ (MSE) 
& \textbf{0.00936} / 0.03943 / 0.35182 / 0.14755 
& \textbf{7.8e-5} / 2.6e-4 / 7.29e-3 / 5.23e-3 
& 0.6925 / 0.9536 / 0.4925 / \textbf{0.4046} \\
\hline
Euler angle error $\gamma$ (MSE) 
& \textbf{0.00930} / 0.04331 / 0.30561 / 0.16116 
& \textbf{6.4e-5} / 1.4e-3 / 3.82e-3 / 2.29e-3 
& 0.5701 / 0.7725 / 0.3833 / \textbf{0.3788} \\
\hline
\end{tabular}
}
\end{table*}



\begin{figure*}
\centering
\includegraphics[width=0.59\linewidth]{wacv-2026-author-kit-template/Results/Without_shifts/Visual_Results_without_results_combined.png}
\includegraphics[width=\linewidth]{wacv-2026-author-kit-template/Results/Without_shifts/FSC_without_shifts_results_combined.png}
\caption{Visual Comparison and FSC curves for SNR 0.1, 1000 particles for 3 different maps.  These results confirm that robust joint pose estimation not only improves angular consistency but also yields higher-quality reconstructions, even in the presence of strong noise. \alertKG{Better to maintain the same color for an algorithm across different maps and use the same color for FSC curves too. For instance, ground truth is pink, ours purple, etc.}
\alertKS{I'll take a look at it after the entire paper is finished, the process is too tedious.}}
\label{fig:joint_opt_validation}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_shift_correction.tex <==
% \section{Introduction to Shift Correction in Cryo-EM}

% Cryo-electron microscopy (Cryo-EM) requires the alignment of 2D projection images to reconstruct high-resolution 3D structures. Each projection image, denoted as \( Q_k \) for \( k = 1, 2, \dots, K \), is shifted relative to its unshifted counterpart \( P_k \). The amount of translation in the \( x \)- and \( y \)-directions for each image is represented by the unknown parameters \( \Delta x_k \) and \( \Delta y_k \), respectively. The ability to accurately estimate these shifts is crucial for reconstructing the 3D structure of the macromolecule. 

% Previous methods, such as those proposed by \cite{Singer2012}, use common-line detection to estimate shifts. However, in the presence of noise, these methods can lead to inconsistencies as the common lines used for shift estimation may change during the iterative process. The challenge is to ensure that the shift estimation process leads to a consistent solution where the common lines are aligned after each correction step.

% In this section, we introduce a refined shift correction procedure designed to ensure consistency in the shift estimation process. The core idea is to iteratively correct the shifts while maintaining consistency across the projections, ensuring that the residuals \( A\mathbf{x} - \mathbf{b} \) converge and saturate, thereby stabilizing the solution.

% \section{The Refined Shift Correction Algorithm}

% The refined shift correction method focuses on ensuring that the solution to the shift estimation problem remains consistent across iterations. This is particularly important because after each correction, the common lines—used to estimate the relative phase shifts—can change, leading to inconsistencies. Our iterative approach addresses this by ensuring that the solution converges and the common lines remain aligned.

% \subsection{Algorithm Overview}

% The refined shift correction algorithm follows a set of iterative steps designed to improve the accuracy and consistency of the estimated shifts:

% \begin{enumerate}
%     \item \textbf{Initial Shift Estimation:} Start by estimating the initial shifts, \( \Delta x_k^{(0)} \) and \( \Delta y_k^{(0)} \), using the Fourier shift theorem. This provides an initial guess for the alignment of the projections.
%     \item \textbf{Iterative Refinement:} For each iteration, apply the estimated shifts to the projections and recompute the common lines. The phase shifts \( \mu_{1,2} \) for each pair of projections are then updated based on the cross-correlation between the common lines. The shifts are re-estimated by solving a least-squares optimization problem.
%     \item \textbf{Consistency Check:} After each iteration, check if the residuals \( A\mathbf{x} - \mathbf{b} \) have converged. This ensures that the shifts are consistent and that the common lines are correctly aligned.
% \end{enumerate}

% \subsection{Definitions of Variables}

% Before proceeding, we define the key variables used in the algorithm:

% \begin{itemize}
%     \item $\mathcal{F}_k(r, \theta)$: Polar Fourier transform of the $k$-th projection image, where $r$ is the radial frequency and $\theta$ is the angle.
%     \item $\Delta x_k, \Delta y_k$: Unknown 2D shifts for the $k$-th projection in Cartesian coordinates.
%     \item $\hat{\mathcal{F}}_k(r, \theta)$: Phase-corrected projection after applying current shift estimates, where $\hat{\mathcal{F}}_k = \mathcal{F}_k \odot \exp(-2\pi i \Phi_k)$ with $\Phi_k(r,\theta) = r[\Delta x_k \sin\theta + \Delta y_k \cos\theta]$.
%     \item $c_1, c_2$: Indices of common lines (matching rays) between two projections in polar coordinates.
%     \item $s^*$: Optimal 1D shift along the common line that maximizes correlation between two rays.
%     \item $\mathbf{A} \in \mathbb{R}^{M \times 2K}$: Sparse matrix encoding the geometry of common lines, where $M = K(K-1)/2$ is the number of projection pairs. Each row of $\mathbf{A}$ corresponds to a pair of projections $(k_1, k_2)$ and contains four nonzero entries: $\sin\alpha$ and $\cos\alpha$ at the indices for $\Delta x_{k_1}$ and $\Delta y_{k_1}$, and $-\sin\beta$ and $-\cos\beta$ at the indices for $\Delta x_{k_2}$ and $\Delta y_{k_2}$, where $\alpha$ and $\beta$ are the angles of the detected common lines in projections $k_1$ and $k_2$ respectively.

%     \item $\mathbf{b} \in \mathbb{R}^M$: Vector of measured 1D shifts $s^*$ between common lines.
%     \item $\mathbf{x} = [\Delta x_1, \Delta y_1, \ldots, \Delta x_K, \Delta y_K]^T \in \mathbb{R}^{2K}$: Vector of all unknown 2D shifts.
% \end{itemize}
% \subsection{Refined Shift Correction Algorithm}

% The refined shift correction algorithm is designed to iteratively update the shift estimates and ensure consistency in the common-line detection process. Here’s how it works:

% % \begin{algorithm}[H]
% % \caption{Refined Shift Correction for Consistent Cryo-EM Projections}
% % \label{alg:shift_refinement}
% % \begin{algorithmic}[1]
% % \State \textbf{Input:} Set of projection images Q \( Q_1, Q_2, \dots, Q_K \) in polar fourier domain
% % \State \textbf{Output:} Refined shifts \( \Delta x_1, \Delta y_1, \dots, \Delta x_K, \Delta y_K \)
% % \State \textbf{Initialize:} Compute initial shifts \( \Delta x_1^{(0)}, \Delta y_1^{(0)}, \dots, \Delta x_K^{(0)}, \Delta y_K^{(0)} \) using \cite{Singer2012}
% % \For{each iteration}
% %     \State Add appropriate phase shifts to the projections Q  with the current estimate of shifts to form \hat{Q}.
% %     \For{each pair of projections \(\hat{Q}_{k_1}, \hat{Q}_{k_2} \)} 
% %         \State Find out the position ($cl_{1}$, $cl_2$) of the common lines (radial lines) in \hat{Q}
        
% %         \State Find the phase shift (b corresponding to current pair of projections) that will maximise the normalized cross-correlation between the radial lines indexed by ($cl_{1}$, $cl_2$) in Q. 
% %     \EndFor
% %     \State Solve the least-squares problem to estimate updated shifts \( \Delta x_1, \Delta y_1, \dots, \Delta x_K, \Delta y_K \)
% %     \State \textbf{Check Consistency:} Check if \( A\mathbf{x} - \mathbf{b} \) has converged.
% %     \EndIf
% % \EndFor
% % \State \Return Refined shifts \( \Delta x_1, \Delta y_1, \dots, \Delta x_K, \Delta y_K \)
% % \end{algorithmic}
% % \end{algorithm}
% \begin{algorithm}[H]
% \caption*{Iterative Shift Refinement for Cryo-EM Projections}
% \label{alg:shift_refinement}
% \begin{algorithmic}[1]
% \Require Projections $\{\mathcal{F}_k\}_{k=1}^K$ in polar Fourier domain, initial shifts $\{(\Delta x_k^{(0)}, \Delta y_k^{(0)})\}_{k=1}^K$
% \Ensure Refined shifts $\{(\Delta x_k, \Delta y_k)\}_{k=1}^K$
% \State Set convergence threshold $\epsilon$, iteration $t = 0$
% \While{not converged}
%     \State $t \leftarrow t + 1$
%     \State 
%     \State \textbf{Step 1: Apply phase corrections}
%     \For{$k = 1$ to $K$}
%         \State $\hat{\mathcal{F}}_k = \mathcal{F}_k \odot \exp(-2\pi i [\Delta x_k^{(t-1)} r\sin\theta + \Delta y_k^{(t-1)} r\cos\theta])$
%     \EndFor
%     \State 
%     \State \textbf{Step 2: Detect common lines and estimate shifts}
%     \State Initialize equation counter $\ell = 0$
%     \For{$k_1 = 1$ to $K-1$}
%         \For{$k_2 = k_1 + 1$ to $K$}
%             \State $(c_1, c_2) = \arg\max$ correlation($\hat{\mathcal{F}}_{k_1}$, $\hat{\mathcal{F}}_{k_2}$)
%             \State $\mathbf{r}_1 = \mathcal{F}_{k_1}(:, c_1)$, $\mathbf{r}_2 = \mathcal{F}_{k_2}(:, c_2)$
%             \State $s^* = \arg\max_s$ correlation($\mathbf{r}_1 \odot e^{-2\pi i s \mathbf{f}}, \mathbf{r}_2$)
%             \State $b_\ell = s^*$
%             \State $\alpha = (c_1-1)\pi/n_\theta$, $\beta = (c_2-1)\pi/n_\theta$
%             \State Add row to $\mathbf{A}$ using $\alpha$, $\beta$
%             \State $\ell \leftarrow \ell + 1$
%         \EndFor
%     \EndFor
%     \State 
%     \State \textbf{Step 3: Solve} $\mathbf{A}\mathbf{x} = \mathbf{b}$ where $\mathbf{x} = [\Delta x_1, \Delta y_1, ..., \Delta x_K, \Delta y_K]^T$
%     \State 
%     \State \textbf{Step 4: Check convergence}
%     \If{$\|\mathbf{A}\mathbf{x} - \mathbf{b}\|_2$ converged}
%         \State \textbf{break}
%     \EndIf
% \EndWhile
% \State \Return $\{(\Delta x_k^{(t)}, \Delta y_k^{(t)})\}_{k=1}^K$
% \end{algorithmic}
% \end{algorithm}
% \begin{itemize}
%     \item \textbf{Phase Correction:} Each projection $\mathcal{F}_k$ is phase-modulated using its current shift estimate to obtain a corrected profile $\hat{\mathcal{F}}_k$, compensating for the assumed translation.
    
%     \item \textbf{Common-Line Matching:} For each pair of projections $(k_1, k_2)$, the most correlated rays $(c_1, c_2)$ are detected using $\hat{\mathcal{F}}_{k_1}$ and $\hat{\mathcal{F}}_{k_2}$. The same ray positions are then extracted from the original (unshifted) projections to estimate the relative translation $s^*$ via 1D phase alignment. These measurements define linear constraints used to construct a global system $\mathbf{A}\mathbf{x} = \mathbf{b}$, where $\mathbf{x}$ encodes all shifts.
    
%     \item \textbf{Least-Squares Update:} The system is solved in the least-squares sense to obtain updated shift estimates.

%     \item \textbf{Convergence Check:} If the residual norm $\|\mathbf{A}\mathbf{x} - \mathbf{b}\|_2$ falls below a threshold or stabilizes, the algorithm terminates; otherwise, the updated shifts are used to repeat the process.
% \end{itemize}

% The algorithm converges when the estimated shifts yield common-line alignments that are consistent across all projection pairs.



% \section{In-Plane Shift Correction via Iterative Common-Line Consistency}

% In Cryo-EM, accurate 3D reconstruction requires aligning 2D projections that may be shifted due to sample drift, beam-induced motion, or particle picking errors. Each observed projection \( Q_k \) is a translated version of its true, centered projection \( P_k \), with unknown in-plane displacements \( (\Delta x_k, \Delta y_k) \). Ignoring these shifts can severely degrade pose estimation and reconstruction.

% Prior work, such as \cite{Singer2012}, estimates shifts by solving a global system derived from pairwise common-line constraints. However, in noisy conditions, these constraints may change after applying estimated shifts, leading to inconsistency. Our method addresses this by enforcing iterative consistency between the estimated shifts and the detected common lines.

% \subsection{Overview of the Shift Refinement Algorithm}

% Given a set of noisy, shifted projection images in the Fourier domain, our goal is to estimate their in-plane translations such that the common-line constraints across projection pairs are jointly satisfied. The proposed method follows an iterative refinement strategy. At each iteration, the current shift estimates are used to phase-correct the projections. Pairwise common lines are then re-estimated by identifying the maximally correlated rays between projections. These matches yield linear equations that relate the unknown shifts to the estimated phase offsets along common lines. The resulting sparse linear system is solved in a least-squares sense to update the shift estimates. This process is repeated until convergence, defined by the stabilization of the residual error or shift updates. By re-aligning projections based on globally consistent common-line geometry, the method ensures that the estimated shifts are geometrically coherent across the dataset.

% \subsection{Variable Definitions}

% \begin{itemize}[noitemsep, topsep=0pt]
%     \item $\mathcal{F}_k(r, \theta)$: Polar Fourier transform of the $k$-th projection.
%     \item $\hat{\mathcal{F}}_k(r, \theta)$: Phase-corrected Fourier slice after applying current shift estimate.
%     \item $(\Delta x_k, \Delta y_k)$: Unknown 2D shifts for projection $k$.
%     \item $(c_1, c_2)$: Best-matching common line indices between two projections.
%     \item $s^*$: Estimated 1D relative shift along the detected common line.
%     \item $\mathbf{x} \in \mathbb{R}^{2K}$: Stack of all $K$ 2D shifts.
%     \item $\mathbf{A} \in \mathbb{R}^{M \times 2K}$: Sparse system matrix ($M = \binom{K}{2}$).
%     \item $\mathbf{b} \in \mathbb{R}^{M}$: Phase shift offsets from pairwise alignment.
% \end{itemize}

% \subsection{Refined Shift Correction Algorithm}

% \vspace{-1mm}
% \begin{algorithm}[H]
% \caption{Iterative Shift Refinement}
% \label{alg:shift_refine}
% \begin{algorithmic}[1]
% \Require Fourier slices $\{\mathcal{F}_k\}_{k=1}^K$, initial shifts $\{(\Delta x_k^{(0)}, \Delta y_k^{(0)})\}$
% \Ensure Refined shifts $\{(\Delta x_k, \Delta y_k)\}_{k=1}^K$
% \State Set convergence threshold $\epsilon$, iteration $t = 0$
% \Repeat
%     \State $t \gets t + 1$
%     \For{$k = 1$ to $K$}
%         \State Apply phase shift to correct projection:
%         \[
%         \hat{\mathcal{F}}_k = \mathcal{F}_k \cdot \exp(-2\pi i [\Delta x_k^{(t-1)} r \sin\theta + \Delta y_k^{(t-1)} r \cos\theta])
%         \]
%     \EndFor

%     \State Initialize sparse matrix $\mathbf{A}$ and vector $\mathbf{b}$

%     \For{$k_1 = 1$ to $K-1$}
%         \For{$k_2 = k_1 + 1$ to $K$}
%             \State Detect most correlated rays $(c_1, c_2)$ in $\hat{\mathcal{F}}_{k_1}, \hat{\mathcal{F}}_{k_2}$
%             \State Extract corresponding rays from original projections:
%             $\mathbf{r}_1, \mathbf{r}_2$
%             \State Estimate shift $s^* = \arg\max_s \text{corr}(\mathbf{r}_1 \cdot e^{-2\pi i s \mathbf{f}}, \mathbf{r}_2)$
%             \State Compute angles: $\alpha = \pi (c_1-1)/n_\theta$, $\beta = \pi (c_2-1)/n_\theta$
%             \State Append row to $\mathbf{A}$ using $[\sin\alpha, \cos\alpha, -\sin\beta, -\cos\beta]$ at indices for $(k_1, k_2)$
%             \State Set corresponding entry in $\mathbf{b}$ to $s^*$
%         \EndFor
%     \EndFor

%     \State Solve least-squares: $\mathbf{x}^{(t)} = \arg\min_{\mathbf{x}} \| \mathbf{A} \mathbf{x} - \mathbf{b} \|_2^2$

% \Until{Residual $\|\mathbf{A} \mathbf{x}^{(t)} - \mathbf{b}\|_2$ converges or stagnates}
% \State \Return final shifts $\mathbf{x}^{(t)}$
% \end{algorithmic}
% \end{algorithm}

% \subsection{Consistency and Convergence}

% At convergence, the refined shifts align projections such that the detected common lines and the phase constraints used to compute them remain mutually consistent. This ensures geometric coherence across the dataset and improves downstream pose and structure recovery.



\section{In-Plane Shift Correction via Iterative Common-Line Consistency}
In cryo-EM, accurate 3D reconstruction requires the alignment of 2D projections that may be shifted due to sample drift, beam-induced motion, or particle picking inaccuracies. Each observed projection image $\Tilde{h}_k$ is a translated version of its centered version $h_k$, with unknown in-plane shifts $(\Delta x_k, \Delta y_k)$. Neglecting these displacements can lead to significant errors in pose estimation and downstream volume reconstruction.
The work in \cite{Singer2012} introduced a method to estimate these shifts by solving a global linear system derived from pairwise common-line constraints. However, under realistic noise levels, these constraints may shift as projections are corrected, leading to inconsistent or unstable solutions. We address this by proposing an iterative refinement framework that maintains consistency between estimated shifts and detected common lines throughout the correction process.

\subsection{Shift Refinement via Common-Line Geometry}

Given a set of shifted projections, our goal is to estimate the in-plane translations such that the common-line geometry across all projection pairs becomes globally consistent. The method proceeds iteratively. In each round, the current shift estimates are used to apply phase corrections in Fourier space, which—by the Fourier shift theorem—is equivalent to translating the projections in real space. After this correction, common lines between projection pairs are re-estimated. Using the angular indices of the matched common lines, we locate the corresponding rays in the original, uncorrected Fourier slices. These rays represent the projection data before any phase correction. We then compute the relative phase offset by identifying the one-dimensional shift that maximizes the correlation between these two rays. This ensures that the shift estimates are driven by the original data, while remaining aligned with the geometry inferred from the corrected domain. The set of estimated offsets across projection pairs forms a linear system that relates the unknown shifts to the observed phase differences. Solving this system in the least-squares sense updates the shift estimates. The process repeats until the solution converges. A formal convergence proof for this procedure is outside the scope of this work, but we have always observed numerical convergence in our experiments. The procedure for shift correction is presented in Alg.~\ref{alg:shift_refine}, which uses several notation that are defined below. 
\begin{itemize}[noitemsep, topsep=0pt]
    \item $\mathcal{F}h_k(r, \theta)$: Polar Fourier transform of $h_k$, the $k$-th particle.
    \item $\hat{\mathcal{F}}h_k(r, \theta)$: Fourier slice after phase correction of $h_k$ using current shift estimates.
    \item $(\Delta x_k, \Delta y_k)$: Unknown 2D in-plane shifts for projection $k$.
    \item $(c_i, c_j)$: Indices of common lines between two projections.
    \item $s^*$: Estimated 1D relative shift along the matched radial line.
    \item $\boldsymbol{x} \in \mathbb{R}^{2K}$: Stacked shift vector containing all $K$ projection shifts.
    \item $\boldsymbol{A} \in \mathbb{R}^{M \times 2K}$: Sparse coefficient matrix, with $M = \binom{K}{2}$ equations.
    \item $\boldsymbol{b} \in \mathbb{R}^{M}$: Observed phase offsets derived from radial-line alignment.
\end{itemize}

\begin{algorithm}
\caption{Iterative In-Plane Shift Refinement}
\label{alg:shift_refine}
\begin{algorithmic}[1]
\State \textbf{Require:} Fourier slices $\{\mathcal{F}h_k\}_{k=1}^K$; initial shifts $\{(\Delta x_k^{(0)}, \Delta y_k^{(0)})\}$ ; number of angular rays $n_\theta$
\State \textbf{Ensure:} Refined shifts $\{(\Delta x_k, \Delta y_k)\}_{k=1}^K$
\State Set convergence threshold $\epsilon$; iteration counter $t \gets 0$
\Repeat
    \State $t \gets t + 1$
    \For{$k = 1$ to $K$}
        \State Apply phase correction:
        \[
        \hat{\mathcal{F}}h_k(r, \theta) \gets \mathcal{F}h_k(r, \theta) \cdot 
        e^{-2\pi \iota r \left( \Delta x_k^{(t-1)} \sin\theta + \Delta y_k^{(t-1)} \cos\theta \right)}
        \]
        
    \EndFor

    \State Initialize sparse matrix $\boldsymbol{A}$ and vector $\boldsymbol{b}$

    \For{$k_1 = 1$ to $K-1$}
    \For{$k_2 = k_1 + 1$ to $K$}
\State Find indices $(c_{k_1}, c_{k_2})$ of common-lines in 
       $\hat{\mathcal{F}}h_{k_1}, \hat{\mathcal{F}}h_{k_2}$
\State Extract corresponding rays $r_{k_1}$, $r_{k_2}$ in $\mathcal{F}h_k$: 
\Statex \hspace{4.2em} $\mathbf{r}_{k_1} = \mathcal{F}h_{k_1}(r, \theta_{c_{k_1}})$, \quad $\mathbf{r}_{k_2} = \mathcal{F}h_{k_2}(r, \theta_{c_{k_2}})$

        % \State Extract corresponding rays $\boldsymbol{r}_1$, $\boldsymbol{r}_2$ \alertKG{How r1, r2 differ from c1, c2?}
        \State $s^* \gets \arg\max_s \, \text{corr}(\boldsymbol{r}_{k_1} \cdot e^{-2\pi \iota s \mathbf{f}}, \boldsymbol{r}_{k_2})$
        \State $\alpha \gets \pi (c_{k_1} - 1)/n_\theta$,\quad
               $\beta \gets \pi (c_{k_2} - 1)/n_\theta$
        \State Append $[\sin\alpha,\, \cos\alpha,\, -\sin\beta,\, -\cos\beta]$ to corresponding row of $\boldsymbol{A}$ at indices $[2k_1,\, 2k_1{+}1,\, 2k_2,\, 2k_2{+}1]$ (all other entries zero)
        \State Append $s^*$ to $\boldsymbol{b}$
    \EndFor
    \EndFor

    \State Solve: $\boldsymbol{x}^{(t)} \gets \arg\min_{\boldsymbol{x}} \| \boldsymbol{A} \boldsymbol{x} - \boldsymbol{b} \|_2^2$
\Until{$\|\boldsymbol{A} \boldsymbol{x}^{(t)} - \boldsymbol{b}\|_2$ converges or $\| \boldsymbol{x}^{(t)} - \boldsymbol{x}^{(t-1)} \|$ is below $\epsilon$}
\State \Return $\boldsymbol{x}^{(t)}$
\end{algorithmic}
\end{algorithm}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{wacv-2026-author-kit-template/Results/WACV Flowchart.png}
    \caption{Full pipeline}
    \label{fig:full-pipeline}
\end{figure*}
\section{Experiments with Synthetic Data}
We evaluated the effectiveness of our joint $\ell_1$-norm based pose estimation on simulated Cryo-EM projections corrupted with noise corresponding to a signal to noise ratio (SNR) of 0.1. In this experiments, the projections were assumed to be centered (no shifts). We simulated projections (at different orientations) of three molecular maps taken from the well known database EMDB at \url{https://www.ebi.ac.uk/emdb/}. The molecular maps were:
\begin{itemize}[noitemsep,topsep=0pt]
    \item \textbf{Map 1 (EMD-3508)} – 80S ribosome, size $260^3 \cite{emd3508_Huter2016}$
    \item \textbf{Map 2 (EMD-42525)} – 80S ribosome, size $648^3 \cite{emd42525_Musalgaonkar2025Reh1}$
    \item \textbf{Map 3 (EMD-22689)} – PTCH1 with nanobody, size $256^3 \cite{emd22689_pnas.2011560117}$
\end{itemize}
We generated 1000 Gaussian-corrupted projections per map and compared our method to the spherical embedding approach (SE) ~\cite{lu2022}, least unsquared deviations (LUD)~\cite{wang2013_lud}, and synchronization-based pose estimation (Sync) ~\cite{Shkolnisky2012_sync}, using standard metrics for angular and reconstruction accuracy.
Table~\ref{tab:synthetic_results} reports errors for dihedral and in-plane angle consistency, in-plane rotation, and Euler angles. Figure~\ref{fig:joint_opt_validation} presents visual comparisons and Fourier Shell Correlation (FSC) curves for three synthetic maps. We observe that reconstructions generated using our joint optimization framework align more closely with the ground truth, both in terms of structural detail and frequency preservation, as indicated by higher FSC values across resolutions. In particular, for Map 3 (EMD-22689), it is clearly visible in Figure~\ref{fig:joint_opt_validation} that our method yields the most accurate 3D reconstruction among all baselines. These results confirm that robust joint pose estimation not only improves angular consistency but also leads to significantly better reconstructions, even under high noise conditions.

We then evaluated our complete pipeline—including both pose estimation and shift correction, shown in Figure ~\ref{fig:full-pipeline}—on three derived molecular maps:
\begin{itemize}[noitemsep,topsep=0pt]
    \item \textbf{Map 1 (EMD-41801)} – Cryo-EM structure of the human nucleosome core particle ubiquitylated at histone H2A lysine 15 in complex with RNF168-UbcH5c (class 2), size $256^3 \cite{emd41801_Qi2024}$
    \item \textbf{Map 2 (EMD-17947)} – Trimeric prM/E spike of Tick-borne encephalitis virus
immature particle, size $300^3 \cite{emd_17947_Maria2024}$
    \item \textbf{Map 3 (EMD-22689)} – PTCH1 with nanobody, size $256^3 \cite{emd22689_pnas.2011560117}$
\end{itemize}
For each map, we simulated 1000 shifted projections corrupted with Gaussian noise, again corresponding to an SNR of 0.1. We compared our full pipeline against a baseline shift correction method combined with three existing angle estimation techniques: spherical embedding (SE)~\cite{lu2022}, the least unsquared deviations (LUD) formulation~\cite{wang2013_lud}, and the synchronization method~\cite{Shkolnisky2012_sync}. As described in Figure~\ref{fig:full_pipeline_validation_synthetic}, our full pipeline—combining robust angle estimation with an improved shift correction procedure—produces reconstructions that exhibit greater structural detail and fidelity to the ground truth. Notably, for Map 1 (EMD-41801), our method preserves fine features more accurately than competing approaches. 
 
\begin{figure*}
\centering
\includegraphics[width=0.65\linewidth]{wacv-2026-author-kit-template/Results/With_shifts/Visual_Results_with_results_combined.png}
\includegraphics[width=\linewidth]{wacv-2026-author-kit-template/Results/With_shifts/FSC_with_results_combined.png}
\caption{Visual Comparison and FSC curves for 1000 particles with random orientation and shift, each at SNR 0.1 for 3 different maps. The results confirm the effectiveness of joint pose estimation and shift correction (Alg.~\ref{alg:PGD} and \ref{alg:shift_refine}; also see Fig.~\ref{fig:full-pipeline}).}
\label{fig:full_pipeline_validation_synthetic}
\end{figure*}

\section{Real Data Experiments with the Full Pipeline}

For real datasets acquired from our Cryo-EM facility, ground-truth 3D maps are not available. To serve as a reference for evaluation, we used high-quality reconstructions obtained from the RELION pipeline, which processes millions of particle images to produce state-of-the-art maps. To mitigate the extreme noise levels inherent in raw single-particle images, we used class-averaged 2D projections as input to all methods. This preprocessing step substantially improves the signal-to-noise ratio (SNR) and enables fairer comparisons.

We tested our pipeline on three distinct datasets:
\begin{itemize}[noitemsep,topsep=0pt]
    \item \textbf{Plasmodium falciparum 80S ribosome} bound to the anti-protozoan drug emetine, consisting of approximately 600 class averages~\cite{wong_empiar_10028}
    \item \textbf{Nucleosome particle}, with 851 class averages
\end{itemize}

As shown in the supplement, most methods—including our proposed approach—produce high-quality reconstructions across datasets. An exception is observed in the nucleosome dataset, where the method of \cite{lu2022} fails to recover a meaningful structure. Overall, the improved SNR due to class averaging allows even baseline methods to perform competitively, highlighting the importance of using more challenging, low-SNR inputs to rigorously evaluate pose estimation robustness.

% \begin{figure*}
% \centering
% \includegraphics[width=0.5\linewidth]{wacv-2026-author-kit-template/Results/Visual_Results_Real_data_combined.png}
% \includegraphics[width=0.8\linewidth]{wacv-2026-author-kit-template/Results/FSC_real_data_combined.png}
% \caption{Visual Comparison and FSC curves for two real datasets, algorithms were run on class averages created from millions of particles.}
% \label{fig:full_pipeline_validation_real}
% \end{figure*}


==> sec/3_experiments.tex <==
\section{Experiments and Validation}
We evaluated the effectiveness of our joint $\ell_1$-norm based pose estimation on simulated Cryo-EM datasets corrupted with heavy noise \textcolor{red}{how much noise?}. Specifically, we use three molecular maps from the well known database EMDB from \url{https://www.ebi.ac.uk/emdb/}. We simulated projections of these macromolecules at different angles and added noise to as to produce a signal-to-noise ratio (SNR) of 0.1:
\begin{itemize}[noitemsep,topsep=0pt]
    \item \textbf{Map 1 (EMD-3508)} – 80S ribosome, size $260^3 \cite{emd3508_Huter2016}$
    \item \textbf{Map 2 (EMD-42525)} – 80S ribosome, size $648^3 \cite{emd42525_Musalgaonkar2025Reh1}$
    \item \textbf{Map 3 (EMD-22689)} – PTCH1 with nanobody, size $256^3 \cite{emd22689_pnas.2011560117}$
\end{itemize}
We generated 1000 Gaussian-corrupted projections per map and comparde our method to the spherical embedding approach (SE) ~\cite{lu2022}, least unsquared deviations (LUD)~\cite{wang2013_lud}, and synchronization-based pose estimation (Sync) ~\cite{Shkolnisky2012_sync}, using standard metrics for angular and reconstruction accuracy.
Table~\ref{tab:synthetic_results} reports errors for dihedral and in-plane angle consistency, in-plane rotation, and Euler angles. Figure~\ref{fig:joint_opt_validation} presents visual comparisons and Fourier Shell Correlation (FSC) curves for three synthetic maps. We observe that reconstructions generated using our joint optimization framework align more closely with the ground truth, both in terms of structural detail and frequency preservation, as indicated by higher FSC values across resolutions. In particular, for Map 3 (EMD-22689), it is clearly visible in Figure~\ref{fig:joint_opt_validation} that our method yields the most accurate 3D reconstruction among all baselines. These results confirm that robust joint pose estimation not only improves angular consistency but also leads to significantly better reconstructions, even under high noise conditions.

We validate our joint optimization method on three ribosomal Cryo-EM maps: EMD-13892 \cite{emd13892_mclaren2023}, EMD-16721 \cite{emd16721_Xing2023}, and EMD-3508 \cite{emd3508_Huter2016}. Simulated projections were used to assess pose recovery accuracy against \cite{lu2022} using: mean absolute errors (MAE) of dihedral $\theta_{ij}$ and in-plane $\phi_{ij}$ angles, angular errors in normal/in-plane vectors, Euler angle MSE, and Fourier Shell Correlation (FSC).

\vspace{0.5em}
\noindent\textbf{Map 1 (EMD-13892):} Our method reduces angular errors by over 50\% and improves Euler angle estimation by up to 78\% (Table~\ref{tab:map1_results}). Fig.~\ref{fig:emd13892_results} shows consistently higher FSC correlation and better structural fidelity in reconstructions.

\begin{table}[h]
\centering
\caption{Performance on EMD-13892}
\label{tab:map1_results}
\scriptsize
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Metric} & \textbf{Standard} & \textbf{Ours} & \textbf{Gain} \\
\hline
MAE $\theta_{ij}$ & 0.3371 & 0.1699 & 50.5\% \\
MAE $\phi_{ij}$ & 0.4712 & 0.2432 & 48.4\% \\
In-plane error ($^\circ$) & 34.27 & 16.98 & 50.4\% \\
Normal vector error ($^\circ$) & 22.45 & 10.50 & 53.2\% \\
Euler MSE ($\alpha$/$\beta$/$\gamma$) & 0.096/0.390/0.814 & 0.026/0.084/0.498 & 73/78/39\% \\
\hline
\end{tabular}
\end{table}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Results/emd_13892_FSC_0.1_without_shifts.png}
    \caption{FSC curves}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Results/Visual_comparison_13892_without_shifts.jpeg}
    \caption{Reconstructions}
\end{subfigure}
\caption{Results for EMD-13892. (a) FSC: ours (yellow), \cite{lu2022} (blue). (b) Visual: GT (pink), ours (blue), baseline (red).}
\label{fig:emd13892_results}
\end{figure*}

\vspace{0.5em}
\noindent\textbf{Map 2 (EMD-16721):} Despite higher base errors, our method achieves up to 48\% gains in Euler MSE and notable improvement in fine-structure recovery (Table~\ref{tab:map2_results}, Fig.~\ref{fig:emd16721_results}).

\begin{table}[h]
\centering
\caption{Performance on EMD-16721}
\label{tab:map2_results}
\scriptsize
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Metric} & \textbf{Standard} & \textbf{Ours} & \textbf{Gain} \\
\hline
MAE $\theta_{ij}$ & 0.4592 & 0.4035 & 12.1\% \\
MAE $\phi_{ij}$ & 0.4050 & 0.3221 & 20.5\% \\
In-plane error ($^\circ$) & 33.14 & 21.84 & 34.1\% \\
Normal vector error ($^\circ$) & 33.76 & 27.81 & 17.6\% \\
Euler MSE ($\alpha$/$\beta$/$\gamma$) & 0.197/1.008/0.821 & 0.155/0.618/0.428 & 21/39/48\% \\
\hline
\end{tabular}
\end{table}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Results/emd_16721_FSC_0.1_without_shifts.png}
    \caption{FSC curves}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Results/Visual_comparison_16721_without_shifts.png}
    \caption{Reconstructions}
\end{subfigure}
\caption{Results for EMD-16721. (a) FSC: ours (yellow), \cite{lu2022} (blue). (b) Visual: GT (blue), ours (orange), baseline (green).}
\label{fig:emd16721_results}
\end{figure*}

\vspace{0.5em}
\noindent\textbf{Map 3 (EMD-3508):} As shown in Table~\ref{tab:map3_results} and Fig.~\ref{fig:emd3508_results}, our method achieves its highest gains here, with up to 86\% improvement in Euler MSE and near-perfect structural recovery.

\begin{table}[h]
\centering
\caption{Performance on EMD-3508}
\label{tab:map3_results}
\scriptsize
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Metric} & \textbf{Standard} & \textbf{Ours} & \textbf{Gain} \\
\hline
MAE $\theta_{ij}$ & 0.0747 & 0.0267 & 64.3\% \\
MAE $\phi_{ij}$ & 0.0795 & 0.0196 & 75.3\% \\
In-plane error ($^\circ$) & 6.56 & 1.56 & 76.2\% \\
Normal vector error ($^\circ$) & 4.74 & 1.59 & 66.5\% \\
Euler MSE ($\alpha$/$\beta$/$\gamma$) & 0.0057/0.039/0.043 & 0.0008/0.009/0.009 & 86/76/79\% \\
\hline
\end{tabular}
\end{table}

\begin{figure*}[h]
\centering
\begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Results/emd_3508_FSC_0.1_without_shifts.jpg}
    \caption{FSC curves}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Results/Visual_comparison_emd3508_without_shifts.jpeg}
    \caption{Reconstructions}
\end{subfigure}
\caption{Results for EMD-3508. (a) FSC: ours (yellow), baseline (blue). (b) Visual: GT (left), ours (middle), baseline (right).}
\label{fig:emd3508_results}
\end{figure*}


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/4_conclusion.tex <==
\section{Conclusion and Future Work}

In this paper, we introduced a robust joint optimization framework for cryo-EM pose estimation that improves upon existing methods in both angular alignment and in-plane shift correction. Our first contribution is a principled $\ell_1$-norm based spherical embedding algorithm that accurately estimates projection directions under high noise conditions, outperforming state-of-the-art approaches such as LUD~\cite{wang2013_lud}, synchronization-based method~\cite{Shkolnisky2012_sync}, and the spherical embedding method of Lu et al.~\cite{lu2022}. The second contribution enhances the shift correction procedure proposed by Singer et al.~\cite{Singer2012} through an iterative refinement strategy that enforces consistency between the common lines and shifts.

\alertKS{Need to mention the limitations of Synchronization and LUD here with a hint for future work in the same.} Our full pipeline, illustrated in Figure~\ref{fig:full-pipeline}, consistently yields more accurate 3D reconstructions across synthetic datasets. However, a key limitation lies in the reliability of common lines created in the iterative shift refinement. In particular, under extreme noise, the common-line matches may degrade in quality compared to those generated by Singer et al.~\cite{Singer2012}. Future work will focus on improving the reliability of common-line detection within our iterative framework and further enhancing robustness to noise.


==> sec/Real_data.tex <==
% \section{Real Data Experiments with the Full Pipeline}

% For real datasets acquired from our Cryo-EM facility, ground-truth 3D maps are not available. To serve as a reference for evaluation, we used high-quality reconstructions obtained from the RELION pipeline, which processes millions of particle images to produce state-of-the-art maps. To mitigate the extreme noise levels inherent in raw single-particle images, we used class-averaged 2D projections as input to all methods. This preprocessing step substantially improves the signal-to-noise ratio (SNR) and enables fairer comparisons.

% We tested our pipeline on three distinct datasets:
% \begin{itemize}[noitemsep,topsep=0pt]
%     \item \textbf{Plasmodium falciparum 80S ribosome} bound to the anti-protozoan drug emetine, consisting of approximately 600 class averages~\cite{wong_empiar_10028}
%     \item \textbf{Nucleosome particle}, with 851 class averages
% \end{itemize}

% As shown in Figure~\ref{fig:full_pipeline_validation_real}, most methods—including our proposed approach—produce high-quality reconstructions across datasets. An exception is observed in the nucleosome dataset, where the method of \cite{lu2022} fails to recover a meaningful structure. Overall, the improved SNR due to class averaging allows even baseline methods to perform competitively, highlighting the importance of using more challenging, low-SNR inputs to rigorously evaluate pose estimation robustness.
\section{Real Data: Raw Particles and Class Averages}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.48\linewidth]{wacv-2026-author-kit-template/Results/Raw_realdata_particle_1.png}
    \includegraphics[width=0.48\linewidth]{wacv-2026-author-kit-template/Results/Raw_realdata_particle_2.png}
    \caption{Example raw particle images extracted from a micrograph. These projections exhibit extremely low signal-to-noise ratio (SNR), making it challenging for pose estimation and reconstruction algorithms—especially those designed to operate with a limited number of particles—to recover meaningful 3D structure.}
    \label{fig:sample_raw_particles}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{wacv-2026-author-kit-template/Results/Class_averages_sample.png}
    \caption{Sample class averages generated by RELION. Each class average represents the mean of thousands of similar particle images, substantially improving the SNR. These noise-reduced projections enable accurate 3D reconstructions even with a small number of input views. However, generating class averages requires acquiring and processing millions of raw particles.}
    \label{fig:sample_class_averages}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.5\linewidth]{wacv-2026-author-kit-template/Results/Visual_Results_Real_data_combined.png}
\includegraphics[width=0.6\linewidth]{wacv-2026-author-kit-template/Results/FSC_real_data_combined.png}
\caption{Visual Comparison and FSC curves for two real datasets, algorithms were run on class averages created from millions of particles.}
\label{fig:full_pipeline_validation_real}
\end{figure*}

